OTA-Key: Over the Air Key Management for Flexible and Reliable IoT Device Provision

As the Internet of Things (IoT) industry advances, the imperative to secure IoT devices has become increasingly critical. Current practices in both industry and academia advocate for the enhancement of device security through key installation. However, it has been observed that, in practice, IoT vendors frequently assign shared keys to batches of devices. This practice can expose devices to risks, such as data theft by attackers or large-scale Distributed Denial of Service (DDoS) attacks. To address this issue, our intuition is to assign a unique key to each device. Unfortunately, this strategy proves to be highly complex within the IoT context, as existing keys are typically hardcoded into the firmware, necessitating the creation of bespoke firmware for each device. Furthermore, correct pairing of device keys with their respective devices is crucial. Errors in this pairing process would incur substantial human and temporal resources to rectify and require extensive communication between IoT vendors, device manufacturers, and cloud platforms, leading to significant communication overhead. To overcome these challenges, we propose the OTA-Key scheme. This approach fundamentally decouples device keys from the firmware features stored in flash memory, utilizing an intermediary server to allocate unique device keys in two distinct stages and update keys. We conducted a formal security verification of our scheme using ProVerif and assessed its performance through a series of evaluations. The results demonstrate that our scheme is secure and effectively manages the large-scale distribution and updating of unique device keys. Additionally, it achieves significantly lower update times and data transfer volumes compared to other schemes.

==> sections/2-Problem.tex <==
\section{Problem Statement and Motivation}

\subsection{Limitations in Existing Device Provision Solutions}
\qian{To provision IoT devices, the industry typically employs two methods. The first method, commonly practiced (\cite{changhong, hisilicon, yiqismart}), involves embedding a same device key (such as X.509 certificates and secrets/passwords) directly into the firmware, which is then installed across devices of the same model. This approach results in many IoT devices sharing the same key, thereby presenting significant security risks if even one device is compromised. The second method involves the IoT vendor assigning a unique key to each device's firmware, compiling the firmware individually, and then transferring it to the Device Manager (DM) for installation on the devices. Although secure, this method is time-consuming and labor-intensive. Moreover, these methods do not consider the need to switch cloud platforms.}

\qian{The approach described by Bovskov et al. (\cite{bovskov2020time}) supports only Bluetooth devices and does not account for heterogeneous cloud platforms. Suzaki et al. (\cite{suzaki2020reboot}) focus primarily on rebooting and recovering compromised devices, without considering the distribution of keys to devices. Both approaches assume that the device key is hardcoded into the device firmware, which prevents the independent updating of device keys.}

\qian{The Intel\textregistered  SDO\cite{intel_sdo} only offers a set of standards without providing specific implementations, making it difficult to evaluate. Furthermore, this standard does not emphasize the necessity of assigning unique keys to each device.}

% \cite{bovskov2020time} 仅支持蓝牙设备，do not consider the heterogeneous cloud platforms \cite{suzaki2020reboot} 关注的重点在对compromised devices进行重启与回收，没有考虑如何为设备分发密钥。这两种方案都假设device key hardcode在设备固件中，无法实现对设备 key的单独更新。
% Intel SDO方案仅提供了一套标准，并没有提供具体的实现。

\subsection{Challenges of Setting Unique Keys for Different Devices}

\textbf{Analysis of workflow.} In the workflow (Fig .\ref{fig:system setting}), assigning a unique device key to each device by the IoT vendor is challenging due to two primary reasons:
\begin{enumerate}
    \item \textbf{\textit{High Communication Costs. }} IoT vendors need to frequently negotiate with Device Manufacturers (DMs) and IoT clouds. As depicted in Fig.\ref{fig:system setting}, the lifecycle of a device encompasses several stages, from inception to firmware installation. This process necessitates that the IoT vendor transmits the compiled firmware to the DM and uploads the corresponding certificates to the IoT cloud platform. Ensuring that the device’s certificates match those on the cloud is crucial for seamless connectivity. While the depicted workflow is simplified, it hints at the complexities involved in real-world scenarios. These often include collaborations between an IoT vendor and multiple DMs, alongside various IoT cloud platforms, thereby increasing the IoT vendors’ communication costs.
    \item \textbf{\textit{Weak Motivation.} }Although IoT vendors allocate keys to devices, in the pursuit of rapid market capture, they often sacrifice a degree of security for faster production ( \cite{el_jaouhari_secure_2022}). Assigning a unique device key within the existing production workflow would require the IoT vendor to transmit firmware to the DM for each device produced. Moreover, the physical capture required for IoT device reverse engineering suggests a perceived safety under surveillance and legal protection. This leads some IoT vendors to prioritize market capture over individual device key allocation due to the intense competition in the IoT market.
\end{enumerate}


% \subsection{Threat Model and Assumptions}

\subsection{The Need for Flexible Key Management}
\label{subsec:need-flexible-key}
\qian{In current production line, the IoT vendor does not account for the need to update the device keys to address issue that device key leakage ( \cite{mosenia_comprehensive_2017}, \cite{el_jaouhari_secure_2022}). Specifically, \cite{el_jaouhari_secure_2022} underscores the security risks arising from IoT vendors compromising on secure production strategies in their rush to rapidly deploy devices. This approach, aimed at increasing market dominance, often results in devices sharing keys,  which further exacerbates the need for key updates. To update device keys within the existing production process, the IoT vendor has to return the device to the DM for firmware re-burning, incurring substantial costs. Furthermore, according to~\cite{draft_swithCloud}, a recent EU draft mandates that IoT devices must be able to easily switch cloud services to prevent large cloud platforms from monopolizing data. This requirement necessitates the updating of device keys.}

% \qian{As studies by El Jaouhari\cite{el_jaouhari_secure_2022}, Mosenia\cite{mosenia_comprehensive_2017}, and Khan\cite{khan_iot_2018} demonstrate, IoT devices are susceptible to a variety of attacks, including those from the Mirai botnet, privacy leaks due to credential exposure, and denial-of-service attacks orchestrated by attackers. These articles stress the importance of timely and rapid firmware updates to patch vulnerabilities in IoT devices to ensure their security. Specifically, \cite{el_jaouhari_secure_2022} highlights the security risks associated with rapid product development aimed at increasing market dominance but compromised by inadequate testing. }

% In current background, the IoT vendor does not account for the need to update the device keys to address issues such as device key leakage, cessation of services by cloud platform vendors, or even the IoT vendor discontinuing its business, necessitating the transfer of the device to another IoT vendor. To implement these requirements within the existing production process, the IoT vendor would need to return the device to the DM for firmware re-burning, incurring substantial costs. \qian{The reasons and requirements for this will be outlined in Subsection \ref{subsec:need-firmware-uodate} \textbf{IoT Device Firmware Update Methods}.} 

% 将在\S~\ref{subsec:need-firmware-uodate}小结说明其原因


==> sections/references.tex <==
\section*{references}


